Continual Learning of Large Language Models: A Comprehensive Survey

The recent success of large language models (LLMs) trained on static, pre-collected, general datasets has sparked numerous research directions and applications. One such direction addresses the non-trivial challenge of integrating pre-trained LLMs into dynamic data distributions, task structures, and user preferences. Pre-trained LLMs, when tailored for specific needs, often experience significant performance degradation in previous knowledge domains -- a phenomenon known as "catastrophic forgetting". While extensively studied in the continual learning (CL) community, it presents new manifestations in the realm of LLMs. In this survey, we provide a comprehensive overview of the current research progress on LLMs within the context of CL. This survey is structured into four main sections: we first describe an overview of continually learning LLMs, consisting of two directions of continuity: vertical continuity (or vertical continual learning), i.e., continual adaptation from general to specific capabilities, and horizontal continuity (or horizontal continual learning), i.e., continual adaptation across time and domains (Section 3). We then summarize three stages of learning LLMs in the context of modern CL: Continual Pre-Training (CPT), Domain-Adaptive Pre-training (DAP), and Continual Fine-Tuning (CFT) (Section 4). Then we provide an overview of evaluation protocols for continual learning with LLMs, along with the current available data sources (Section 5). Finally, we discuss intriguing questions pertaining to continual learning for LLMs (Section 6). The full list of papers examined in this survey is available at https://github.com/Wang-ML-Lab/llm-continual-learning-survey.

==> tables/cites_in_figure_left.tex <==
% all the citations to appear in the figure. 
% CPT text boxes
\placetextbox{0.377}{0.818}{\tiny{\cite{loureiro2022timelms,jang2022towards,jin2022lifelong,jang2022temporalwiki,amba2021dynamic,dhingra2022time,yildiz2024investigating}}} % Temporal Shift
\placetextbox{0.532}{0.818}{\tiny{\cite{gupta2023continual,ke2022continual-train,jin2022lifelong,sun2020ernie,cossu2022continual,gururangan2022demix,qin2023recyclable,chen2023lifelong,qin2022elle,ibrahim2024simple}}} % Content Shift
\placetextbox{0.669}{0.818}{\tiny{\cite{gogoulou2024continual,li2024examining,ibrahim2024simple}}} % Language

% DAP text boxes
\placetextbox{0.49}{0.7893}{\tiny{\cite{Lu2023BBTFin,Nguyen2023AstroLLaMA,xie2023efficient,li2023starcoder,guo2024deepseekcoder,Xue2023WeaverBird,paul2024ircoder,cheng2024adapting,dou2024sailor,fujii2024continual,takahashi2024pretraining}}} % DAP
\placetextbox{0.5}{0.7694}{\tiny{\cite{li2023cfgpt,deng2023learning,han2021econet,zhou2020pre,guo2023continuous,gururangan2020dont,yan2023af,rongali2021continual,ma2023ecomgptct}}} % DAP -> SFT
\placetextbox{0.7}{0.7694}{\tiny{\cite{luo2023biomedgpt}}} % DAP -> MM-SFT
\placetextbox{0.792}{0.7694}{\tiny{\cite{wu2024llama}}} % DAP -> U-SFT

\placetextbox{0.475}{0.7486}{\tiny{\cite{Bi2023OCEANGPT,wu2023pmc,Yang2023PLLaMa,li2024blade,xie2024me,nakamura2024aurora}}} % DAP -> IT
\placetextbox{0.62}{0.7486}{\tiny{\cite{Zheng2023MarineGPT}}} % DAP -> MM-IT
\placetextbox{0.71}{0.7486}{\tiny{\cite{colombo2024saullm7b}}} % DAP -> U-IT


\placetextbox{0.475}{0.7284}{\tiny{\cite{song2024code,lin2023geogalactica,rozière2024code,Chen2023HuatuoGPTII,Zhang2023xuanyuan,huang2023lawyer,thulke2024climategpt,acikgoz2024hippocrates}}} % Others
\placetextbox{0.45}{0.7077}{\tiny{\cite{nijkamp2022codegen}}} % DAP -> DAP
\placetextbox{0.57}{0.7077}{\tiny{\cite{ke2022continual-pre}}} % (DAP)_n

% CFT text boxes
\placetextbox{0.416}{0.661}{\tiny{\cite{scialom2022fine,wang2023trace,mok2023large,zhang2023citb,huang2024mitigating}}} % CIT
\placetextbox{0.416}{0.668}{\tiny{\cite{he2024dont,yin2022contintin,wang2023orthogonal,zhao2024sapt}}} % CIT
\placetextbox{0.515}{0.661}{\tiny{\cite{lin2022continual,hartvigsen2023aging,hu2024wilke,wang2024wise}}} % CMR
\placetextbox{0.515}{0.668}{\tiny{\cite{das2024larimar,yu2023melo,li2023continual}}} % CMR
\placetextbox{0.587}{0.661}{\tiny{\cite{zhang2023copf,zhangcppo}}} % CMA
\placetextbox{0.587}{0.668}{\tiny{\cite{lin2024mitigating}}} % CMA
\placetextbox{0.653}{0.661}{\tiny{\cite{he2023continual,zheng2024antiforgetting,chen2024coin}}} % CMLLMs
\placetextbox{0.653}{0.668}{\tiny{\cite{zhu2024model,zhao2024reconstruct}}} % CMLLMs

==> tables/cpt-big.tex <==
% \begin{sidewaystable} % final form of the table.
\begin{landscape}
\begin{table*}[t]
    \centering
    \caption{
    \textbf{Summary of the existing studies on Horizontal Continual Pre-Training of LLMs,} where the papers are organized in the chronological order. 
    In the table, \emph{Dist.~Shift} denotes what type(s) of distributional shifts the study considers and is dedicated to solve, including (i)~temporal shift, (ii)~content shift, and (iii)~language shift.$^1$
    In the section of \textbf{Continual Learning Techniques}$^2$, we mainly categorize three types of continual learning techniques that are studied in the paper: \emph{Rehearsal}, \emph{Parameter Regularization}, and \emph{Architecture Expansion}. 
    We use ``\cmark'', ``\xmark'', and ``\club'' to denote ``deployed in the proposed method'', ``not studied in the paper'', and ``studied as a baseline method'', respectively.
    It is noteworthy that we do not include naive sequential fine-tuning in this table, as it is universally studied as the most important baseline method in all of the papers we investigate. 
    The papers with only ``\club''~\cite{jin2022lifelong,jang2022temporalwiki,jang2022towards} means that merely existing CL techniques are studied in them, and the papers with only ``\xmark''~\cite{gupta2023continual,gogoulou2024continual} means that no CL techniques but special aspects of fine-tuning are studied, e.g., model (re)warming via learning rate scheduling~\cite{gupta2023continual}.
    }
    \label{tab:cpt-big}
    \resizebox{1\linewidth}{!}{%
\begin{tabular}{ccccc ccccc ccccc cc}
	\toprule
	\multirow{3}{*}{\textbf{Method}} & 
    \multicolumn{2}{c}{\textbf{Scenario}} & 
    \multicolumn{10}{c}{\textbf{{Continual Learning Techniques}}} & 
    \multirow{3}{*}{\textbf{{LLM Arch.}}} & 
    \multicolumn{3}{c}{\textbf{{Evaluation}}} \\
    \cmidrule(lr){2-3}\cmidrule(lr){4-13}\cmidrule(lr){15-17}
    & \multirow{2}{*}{\emph{Dist. Shift}} & \multirow{2}{*}{\emph{\#Domains}} &  \multicolumn{3}{c}{\emph{Rehearsal}} &  \multicolumn{2}{c}{\emph{Parameter Regularization}} &  \multicolumn{5}{c}{\emph{Architecture Expansion}} & &  \multicolumn{2}{c}{\emph{Pre-Training}} & \emph{Downstream} \\
    \cmidrule(lr){4-6}\cmidrule(lr){7-8}\cmidrule(lr){9-13}\cmidrule(lr){15-16}\cmidrule(lr){17-17}
    & & & \small{ER} & \small{KD} & \small{Pseudo-ER} & \small{Param. Freezing} & \small{Imp.-based Reg.} & \small{Vocab. Exp.} & \small{Prompt Tuning} & \small{Layer Exp.} & \small{LoRA} & \small{Adapter} & & \small{Perp.} & \small{ZS/FS} & \small{FT Perf.}\\
	%  &
    \midrule
    \midrule
    \cite{sun2020ernie} & Content & 4 & \cmark\club & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & ERNIE & \xmark & \xmark & \cmark \\
    \midrule
	\cite{amba2021dynamic} & Temporal & 7 & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark &  BERT & \xmark & \xmark & \cmark \\
    \midrule
    \cite{cossu2022continual} & Content & 5 & \xmark & \xmark & \xmark & \xmark  & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \makecell{BERT \& \\ RoBERTa} & \xmark & \xmark & \cmark\\
    \midrule
    % \cite{jin2022lifelong}  & \makecell{\underline{Temporal} \\ Content} & \makecell{\underline{4} \\ 8} & \club & \club & \xmark & \xmark & \club & \xmark & \xmark & \club & \xmark & \club & RoBERTa & \cmark & \xmark & \cmark \\
    \multirow{2}{*}{\cite{jin2022lifelong}} & Temporal & 4 & \multirow{2}{*}{\club} & \multirow{2}{*}{\club} & \multirow{2}{*}{\xmark} & \multirow{2}{*}{\xmark} & \multirow{2}{*}{\club} & \multirow{2}{*}{\xmark} & \multirow{2}{*}{\xmark} & \multirow{2}{*}{\club} & \multirow{2}{*}{\xmark} & \multirow{2}{*}{\club} & \multirow{2}{*}{RoBERTa} & \multirow{2}{*}{\cmark} & \multirow{2}{*}{\xmark} & \multirow{2}{*}{\cmark} \\
    \cmidrule(lr){2-3}
    & Content & 8 \\
    \midrule
    \cite{gururangan2022demix} & Content & 8 & \xmark &\xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & GPT-3 & \cmark & \xmark & \cmark \\
    \midrule
    \cite{dhingra2022time} & Temporal & 1 & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark &  \xmark & \xmark & \xmark & \xmark & T5 & \xmark & \xmark & \cmark \\
    \midrule
    \cite{jang2022towards} & Temporal & 1 & \club & \xmark & \xmark & \club & \club & \xmark & \xmark & \xmark & \club & \club & T5 & \xmark & \cmark & \cmark \\
    \midrule
    \cite{jang2022temporalwiki} & Temporal & 5 & \club & \xmark & \xmark & \club & \club & \xmark & \xmark & \xmark & \club & \club & GPT-2 & \cmark & \cmark & \cmark \\
    \midrule
    \cite{qin2022elle} & Content & 5 & \cmark\club & \club & \xmark & \cmark & \club & \xmark & \cmark & \cmark & \xmark & \club & \makecell{BERT \& \\ GPT} & \cmark & \xmark & \cmark \\
    \midrule
    \cite{ke2022continual-train} & Content & 4 & \club & \club & \xmark & \club & \cmark\club & \xmark & \club & \xmark & \xmark & \club & RoBERTa & \xmark & \cmark & \xmark \\
    \midrule
    \cite{qin2023recyclable} & Content & 4 & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & RoBERTa  & \xmark & \xmark & \cmark\\
    \midrule
    \cite{chen2023lifelong} & Content & 3 & \club & \cmark & \xmark & \cmark & \club & \xmark & \xmark & \xmark & \xmark & \cmark & GLaM & \cmark & \xmark & \cmark\\
    \midrule
    \cite{gupta2023continual}  & Content & 1 & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & Pythia & \cmark & \xmark & \xmark \\
    \midrule
    \cite{gogoulou2024continual} & Language & 3 & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & GPT & \cmark & \xmark & \xmark \\
    \midrule
    \cite{li2024examining} & Language & 1 & \xmark & \xmark & \xmark & \club & \xmark & \xmark & \xmark & \xmark & \club & \club & Llama2 & \xmark & \cmark & \cmark \\
	\bottomrule
	\end{tabular}
	}
\end{table*} 
\footnotetext[1]{We provide some examples to better illustrate different types of distributional shifts. \emph{Temporal Shift}: news in year 2021~$\rightarrow$~ news in year 2022; \emph{Content Shift}: papers in chemistry~$\rightarrow$~papers in biology; \emph{Language Shift}: corpus in English~$\rightarrow$~corpus in Chinese.}
\footnotetext[2]{For more information about the categorization of different continual learning techniques, we refer the readers to the work \emph{``A Comprehensive Survey of Continual Learning: Theory, Method and Application''}~\cite{wang2024comprehensive}.}
\footnotetext[3]{In \cite{ke2022continual-train}, the evaluation of the LLMs after domain-adaptive pre-training is carried out following \cite{gu2022ppt}: prompt tuning for few-shot learning, categorized as \emph{ZS / FT}. Although the authors of the original paper categorized their work in ``domain-adaptive pre-training'', sequentially pre-training the LLMs on different topics of domains is considered as continual pre-training.}
\end{landscape}
